The IGRINS YSO Survey III: Stellar parameters of pre-main sequence stars in Ophiuchus and Upper Scorpius

We used the Immersion GRating Infrared Spectrometer (IGRINS) to determine fundamental parameters for 61 K- and M-type young stellar objects (YSOs) located in the Ophiuchus and Upper Scorpius star-forming regions. We employed synthetic spectra and a Markov chain Monte Carlo approach to fit specific K-band spectral regions and determine the photospheric temperature ($T_{\rm eff}$), surface gravity ($\log$ g), magnetic field strength (B), projected rotational velocity ($v \sin i$), and K-band veiling ($r_{\rm K}$). We determined B for $\sim$46% of our sample. Stellar parameters were compared to the results from Taurus-Auriga and the TW Hydrae Association (TWA) presented in Paper I of this series. We classified all the YSOs in the IGRINS survey with infrared spectral indices from 2MASS and WISE photometry between 2 and 24~$\mu$m. We found that Class II YSOs typically have lower $\log$ g and $v\sin i$, similar B, and higher K-band veiling than their Class III counterparts. Additionally, we determined the stellar parameters for a sample of K and M field stars also observed with IGRINS. We have identified intrinsic similarities and differences at different evolutionary stages with our homogeneous determination of stellar parameters in the IGRINS YSO Survey. Considering $\log$ g as a proxy for age, we found that the Ophiuchus and Taurus samples have a similar age. We also find that Upper Scorpius and TWA YSOs have similar ages, and are more evolved than Ophiuchus/Taurus YSOs.

==> tab-zero.tex <==
\begin{deluxetable}{lrrc}
\tablewidth{0pt}
 \tablecaption{Central wavelengths, zero magnitude flux densities, and extiction laws used in this work.\label{tab:zero}}
\tablehead{ \colhead{Band} & \colhead{$\lambda_{\rm c}$} & \colhead{$F_{\nu 0}$} & \colhead{A_\lambda/A$_{K_s}$} \\
\colhead{}& \colhead{($\mu$m)} & \colhead{(Jy)} & \colhead{}}
\startdata 
$J$ & 1.25  &1594 & 2.50\\
$H$ & 1.65  &1024 & 1.55\\
$K_{\rm s}$ & 2.15  &666.7& 1.00 \\
$W1$ & 3.4  &309.54 & 0.79\\
$W2$ & 4.6  &171.787 & 0.55\\
$W3$ & 12.0 &31.674 & 0.61\\
$W4$ & 22.0 &8.363 & 0.43\\
\enddata
\end{deluxetable}
